Electronic and structural properties of crystalline and amorphous (TaNbHfTiZr)C from first principles

High entropy materials (HEMs) are of great interest for their mechanical, chemical and electronic properties. In this paper we analyse (TaNbHfTiZr)C, a carbide type of HEM, both in crystalline and amorphous phases, using density functional theory (DFT). We find that the relaxed lattice volume of the amorphous phase is larger, while its bulk modulus is lower, than that of its crystalline counterpart. Both phases are metallic with all the transition metals contributing similarly to the density of states (DOS) close to the Fermi level, with Ti and Nb giving the proportionally largest contribution of states. We confirm that despite its great structural complexity, 2x2x2 supercells are large enough for reliable simulation of the presented mechanical and electronic properties by DFT.

==> bibliography_roland_and_Tade.tex <==
1	C. Suryanarayana and A. Inoue, Bulk Metallic Glasses, CRC press, 2017. \newline
2	M. M. Trexler and N. N. Thadhani, Mechanical Properties of Bulk Metallic Glasses, Progress in Materials Science, 2010, 55, 759-839. \newline
3	O. Hunderi, Optical Properties of Disordered and Amorphous Metal Films, Thin Solid Films, 1976, 37, 275-280.\newline
4	Z. H. Stachurski, On Structure and Properties of Amorphous Materials, Materials, 2011, 4, 1564-1598.\newline
5	J. R. Scully, A. Gebert and J. H. Payer, Corrosion and Related Mechanical Properties of Bulk Metallic Glasses, Journal of Materials Research, 2007, 22, 302-313.\newline
6	K. Asami, K. Hashimoto, T. Masumoto and S. Shimodaira, ESCA Study of the Passive Film on an Extremely Corrosion-Resistant Amorphous Iron Alloy, Corrosion Science, 1976, 16, 909-914. \newline
7	H. S. Chen, Glassy Metals, Reports on Progress in Physics, 1980, 43, 353-432. \newline
8	J. J. Gilman, Metallic Glasses, Science, 1980, 208, 856-861. \newline
9	J. C. Barbour, F. W. Saris, M. Nastasi and J. W. Mayer, Amorphous Ni-Zr Alloys as Barriers for Self-Diffusion, Physical Review B, 1985, 32, 1363-1365. \newline
10 Cantor B. and Chang I. T. H. and Knight P. and Vincent A. J. B.  Microstructural development in equiatomic multicomponent alloys.  Mater. Sci. Eng. A.  2004;375-377:213-218\newline
11 Yeh J.-W. and Chen S.-K. and Lin S.-J. and Gan J.-Y. and Chin T.-S. and Shun T.-T. and Tsau C.-H. and Chang S.-Y.  Nanostructured High-Entropy Alloys with Multiple Principal Elements: Novel Alloy Design Concepts and Outcomes.  Adv. Eng. Mater.  2004;6(5):299-303 \newline
12 Oses C., Toher C. and Curtarolo S.  High-Entropy Ceramics, Nature Reviews Materials, 2020, 5, 295-309. \newline
13 George P. E., Raabe D. and Ritchie R. O.  High-Entropy Alloys, Nature Reviews Materials, 2019, 4, 515-534. \newline
14 Harrington T. J. et al.  Phase stability and mechanical properties of novel high entropy transition metal carbides.  Acta Materialia, 2019, 166, 271-280. \newline
15 Sarker P.  et al.  High-entropy high-hardness metal carbides discovered by entropy descriptors.  Nature Communications, 2018, 9:4980, 1-10. \newline
16 Wang Y. et al.  Enhanced Hardness in High-Entropy Carbides through Atomic Randomness.  Adv. Theory Simul, 2020,3:2000111, 1-8. \newline
17 Yan X. et al.  (Hf$_{0.2}$Zr$_{0.2}$Ta$_{0.2}$Nb$_{0.2}$Ti$_{0.2}$)C high entropy ceramics with low thermal conductivity. J. Am. Ceram. Soc.  2018:101:4486-4491. \newline
18 Kaloyeros A. and Hoffman M. and William S. W.  Amorphous transition metal carbides, Thin Solid Films, 1986, 2, 237-250. \newline
19 Voevodin A. A. and Prasad S. V. and Zabinski J. S.  Nanocrystalline carbide/amorphous carbon composites. J. Appl. Phys. 1997;82:855-858 \newline
20 Sánchez-López J. C. and Martínez-Martínez D. and López-Cartes C. and Fernández A.  Tribological behaviour of titanium carbide/amorphous carbon nanocompositie coatings: from macro to the micro-scale.  Surf. Coat. Technol.  2008;202:4011-4018 \newline
21 Bi F. and Peng L. and Yu P. and Lai X.  Multilayered Zr-C/a-C film on stainless steel 316L as bipolar plates for proton exchange membrane fuel cells.  J. Power Sources.  2016;314:58-65 \newline
22 Jansson U. and Lewin E.  Sputter deposition of transition-metal carbide films — A critical review from a chemical perspective.  Thin Solid Films.  2013;536:1-24 \newline
23 Folkenant M.  Synthesis and Characterization of Amorphous Carbide-based Thin Films. 2015. Uppsala Universitat. \newline
24 Andersson M. and Urbonaite S. and Lewin E. and Jansson U.  Magnetron sputtering of Zr-Si-C thin films.  Thin Solid Films.  2012;520(20):6375-6381 \newline
25 Nedfors N. and Tengstrand O. and Flink A. and Eklund P. and Hultman L. and Jansson U.  Characterization of amorphous and nanocomposite Nb-Si-C thin films deposited by DC magnetron sputtering.  Thin Solid Films.  2013;545:272-278 \newline
26 Kádas K. et al.  Structural properties of amorphous metal carbides: Theory and experiment.  Acta Mater.  2012;60(12):4720-4728\newline
27 Yang Y. and Wang W. and Gan G.-Y. and Shi X.-F. and Tang B.-Y.  Structural, mechanical and electronic properties of (TaNbHfTiZr)C high entropy carbide under pressure: Ab initio investigation.  Phys. B: Condens. Matter.  2018;550(1):163-170 \newline

==> z_new_references_on_amorphous_films.tex <==
1. Amorphous phase forming ability in(W–C)-based sputtered films

@article{trindade_amorphousWC_1998,
    title = {Amorphous phase forming ability in (W-C)-based sputtered films},
    volume = {46},
    issn = {5},
    shorttitle = {},
    url = {https://www-sciencedirect-com.proxy.uba.uva.nl/science/article/pii/S1359645497003364},
    doi = {https://doi.org/10.1016/S1359-6454(97)00336-4},
    abstract = {The effect of adding transition metals, Me, to the structure of (W–C)-based films obtained by sputtering has been studied by the means of electron probe microanalysis (EPMA), secondary ion mass spectrometry (SIMS), low angle X-ray diffraction (XRD), hot stage transmission electron microscopy (TEM), Mössbauer spectroscopy, extended X-ray absorption fine structure (EXAFS), magnetic measurements and differential thermal analysis (DTA). The results obtained for the films in the as-deposited conditions show two types of structures with different degrees of structural order. Films with Ti, Cr or Au are crystalline with a metastable structure of β-(W,Me)C1-x with 1-x extending from near unity down to about 0.6. In opposition to these, films with Me=Group VIIIA transition metal, show crystalline→amorphous state transitions for Me percentages in the range 5–10 at.\%. The structure of these films consists of small β-MC1-x crystallites with a size of a few unity cells, surrounded by a disordered phase rich in element Me. Concerning the results obtained at increasing temperatures, the chemical and structural behaviour of the W–Me–C films depend on the affinity of carbon for the element Me. Strong or moderate carbide-forming elements (Ti or Cr) improve the stability of the crystalline phase at high temperatures; the films formed by W, C and a weak or non carbide-forming metal (Fe, Co, Ni, Pd or Au) change structurally in the temperature range studied.},
    urldate = {2021-12-6},
    journal = {Acta Materialia},
    author = {Trindade, B and Vieira, M. T. and Bauer-Grosse, E},
    month = mar,
    year = {1998},
    pages = {1731-1739},
    file = {}
}

2. Electronic structure and chemical bonding of amorphous chromium carbide thin films

@article{magnuson_amorphousCrC_2012,
    title = {Electronic structure and chemical bonding of amorphous chromium carbide thin films},
    volume = {24},
    issn = {22},
    shorttitle ={},
    url = {https://iopscience-iop-org.proxy.uba.uva.nl/article/10.1088/0953-8984/24/22/225004},
    doi = {https://doi.org/10.1088/0953-8984/24/22/225004},
    abstract = {The microstructure, electronic structure and chemical bonding of chromium carbide thin films with different carbon contents have been investigated with high-resolution transmission electron microscopy, electron energy loss spectroscopy and soft x-ray absorption–emission spectroscopies. Most of the films can be described as amorphous nanocomposites with non-crystalline CrCx in an amorphous carbon matrix. At high carbon contents, graphene-like structures are formed in the amorphous carbon matrix. At 47 at.\% carbon content, randomly oriented nanocrystallites are formed creating a complex microstructure of three components. The soft x-ray absorption–emission study shows additional peak structures exhibiting non-octahedral coordination and bonding.},
    urldate = {2021-12-6},
    journal = {Journal of Physics: Condensed Matter},
    author = {Magnuson, Martin and Andersson, Matilda and Lu, Jun and Hultman, Lars and Jansson, Ulf},
    month = may,
    year = {2012},
    pages = {225004},
    file = {}
}
  
    3. Structure and bonding in amorphous iron carbide thin films
    https://iopscience-iop-org.proxy.uba.uva.nl/article/10.1088/0953-8984/27/4/045002


@article{furlan_amorphousFeC_2015,
    title = {Structure and bonding in amorphous iron carbide thin films},
    volume = {27},
    issn = {4},
    shorttitle ={},
    url = {https://iopscience-iop-org.proxy.uba.uva.nl/article/10.1088/0953-8984/27/4/045002},
    doi = {https://doi.org/10.1088/0953-8984/27/4/045002},
    abstract = {We investigate the amorphous structure, chemical bonding, and electrical properties of magnetron sputtered Fe1−xCx (0.21 ⩽ x ⩽ 0.72) thin films. X-ray, electron diffraction and transmission electron microscopy show that the Fe1−xCx films are amorphous nanocomposites, consisting of a two-phase domain structure with Fe-rich carbidic FeCy, and a carbon-rich matrix. Pair distribution function analysis indicates a close-range order similar to those of crystalline Fe3C carbides in all films with additional graphene-like structures at high carbon content (71.8 at\% C). From x-ray photoelectron spectroscopy measurements, we find that the amorphous carbidic phase has a composition of 15–25 at\% carbon that slightly increases with total carbon content. X-ray absorption spectra exhibit an increasing number of unoccupied 3d states and a decreasing number of C 2p states as a function of carbon content. These changes signify a systematic redistribution in orbital occupation due to charge-transfer effects at the domain-size-dependent carbide/matrix interfaces. The four-point probe resistivity of the Fe1−xCx films increases exponentially with carbon content from ∼200 μΩ cm (x = 0.21) to ∼1200 μΩ cm (x = 0.72), and is found to depend on the total carbon content rather than the composition of the carbide. Our findings open new possibilities for modifying the resistivity of amorphous thin film coatings based on transition metal carbides through the control of amorphous domain structures.},
    urldate = {2021-12-6},
    journal = {Journal of Physics: Condensed Matter},
    author = {Furlan, Andrej and Jansson, Ulf and Lu, Jun and Hultman, Lars and Magnuson, Martin},
    month = jan,
    year = {2015},
    pages = {045002},
    file = {}
}

    4. Structural, mechanical and electrical-contact properties of nanocrystalline-NbC/amorphous-C coatings deposited by magnetron sputtering
	https://www.sciencedirect.com/science/article/abs/pii/S0257897211007055
	https://doi.org/10.1016/j.surfcoat.2011.07.021

@article{nedfors_nanocrystallineNbC_2011,
    title = {Structural, mechanical and electrical-contact properties of nanocrystalline-NbC/amorphous-C coatings deposited by magnetron sputtering},
    volume = {206},
    issn = {2-3},
    shorttitle ={},
    url = {https://www.sciencedirect.com/science/article/abs/pii/S0257897211007055},
    doi = {https://doi.org/10.1016/j.surfcoat.2011.07.021},
    abstract = {Niobium-carbide nanocomposite coatings with a carbon content varying from 43 to 64 at.\% were deposited by dual DC magnetron sputtering. X-ray diffraction, x-ray photoelectron spectroscopy and electron microscopy showed that all coatings consisted of nanometer sized NbC grains embedded in a matrix of amorphous carbon. Mechanical properties and electrical resistivity showed a strong dependency on the amount of amorphous carbon (a-C) and NbC grain size in the coating. The highest hardness (23 GPa), elastic modulus (295 GPa) and the lowest resistivity (260 μΩ cm) were measured for the coating with about 15\% of a-C phase. Contact resistance measurements using a crossed cylinder set-up showed lowest contact resistance for the coating containing 33\% a-C (140 μΩ at a contact force of 100 N), which is comparable to a Ag reference (45 μΩ at a contact force of 100 N). Comparison with TiC-based nanocomposites studied under similar conditions showed that the Nb-C system has less tendency to form a-C and that lowest contact resistance is obtained at comparable amounts of a-C phase in both material systems (33\% for Nb-C compared to 35\% for Ti-C). With these good electrical contact properties, the Nb-C nanocomposites can be considered as a potential material for electrical contact applications.},
    urldate = {2021-12-6},
    journal = {Surface and Coatings Technology},
    author = {Nedfors, Nils and Tengstrand, Olof and Lewin, Erik and Furlan, Andrej, and Eklund, Per and Hultman, Lars and Jansson, Ulf},
    month = oct,
    year = {2011},
    pages = {354-359},
    file = {}
}

    5. Structure and Bonding in Amorphous Cr1–xCx Nanocomposite Thin Films: X-ray Absorption Spectra and First-Principles Calculations
	https://doi.org/ 10.1021/acs.jpcc.6b03608

@article{olovsson_amorphousCrCXAS_2016,
    title = {Structure and Bonding in Amorphous Cr_{1-x}C_x Nanocomposite Thin Films: X-ray Absorption Spectra and First-Principles Calculations},
    volume = {120},
    issn = {23},
    shorttitle ={},
    url = {https://pubs.acs.org/doi/10.1021/acs.jpcc.6b03608},
    doi = {https://doi.org/10.1021/acs.jpcc.6b03608},
    abstract = {The local structure and chemical bonding in two-phase amorphous Cr1–xCx nanocomposite thin films are investigated by Cr K-edge (1s) X-ray absorption near-edge structure (XANES) and extended X-ray absorption fine structure (EXAFS) spectroscopies in comparison to theory. By utilizing the computationally efficient stochastic quenching (SQ) technique, we reveal the complexity of different Cr-sites in the transition metal carbides, highlighting the need for large scale averaging to obtain theoretical XANES and EXAFS spectra for comparison with measurements. As shown in this work, it is advantageous to use ab initio theory as an assessment to correctly model and fit experimental spectra and investigate the trends of bond lengths and coordination numbers in complex amorphous materials. With sufficient total carbon content (≥30 at. \%), we find that the short-range coordination in the amorphous carbide phase exhibit similarities to that of a Cr7C3 ± y structure, while excessive carbons assemble in the amorphous carbon phase.},
    urldate = {2021-12-6},
    journal = {Journal of Physical Chemistry C},
    author = {Olovsson, Weine and Alling, Björn and Magnuson, Martin},
    month = may,
    year = {2016},
    pages = {12890-12899},
    file = {}
}

    6. Microstructure evolution, wear and corrosion resistance of Cr-C nanocomposite coatings in seawater
	https://doi.org/10.1016/j.apsusc.2018.06.248

@article{zhao_corrosionResistanceCrC_2018,
    title = {Microstructure evolution, wear and corrosion resistance of Cr-C nanocomposite coatings in seawater},
    volume = {457},
    issn = {1},
    shorttitle ={},
    url = {https://www.sciencedirect.com/science/article/abs/pii/S0169433218318154},
    doi = {https://doi.org/10.1016/j.apsusc.2018.06.248},
    abstract = {CrC nanocomposite coatings were deposited by multi-arc ion plating with various argon/acetylene mixtures. The XRD, XPS and HRTEM characterization suggest that the coatings consist of a carbide phase and an amorphous carbon-rich phase. The carbide phase is shown to be CrC with a fcc NaCl (B1) structure. Experiment findings and theoretical calculations reveal phase segregation of sp2-carbon from carbides in which the excess amounts of carbon are incorporated. Nanoindentation, scratch test and Rockwell indentation were performed to investigate the toughness and adhesion ability. A significant improvement of adhesion and toughness is achieved by increasing C content at the expense of hardness. The wear resistance of CrC coatings is controlled by the friction rather than hardness. Compared to dry friction, lower friction coefficients but higher wear rates were obtained under seawater condition. The corrosion behavior of CrC nanocomposite coatings with different C \% was determined by potentiodynamic polarization test and electrochemical impedance spectroscopy (EIS). The coatings with higher Cr content display excellent anti-corrosion properties in seawater.},
    urldate = {2021-12-6},
    journal = {Applied Surface Science},
    author = {Zhao, Daqiang and Jiang, Xin and Wang, Yongxin and Duan, Wenshan and Wang, Liping},
    month = nov,
    year = {2018},
    pages = {914-924},
    file = {}
}

    7. Electronic structure and chemical bonding of nanocrystalline-TiC/amorphous-C nanocomposites
	journals.aps.org/prb/pdf/10.1103/PhysRevB.80.235108
@article{magnuson_TiC_2009,
    title = {Electronic structure and chemical bonding of nanocrystalline-TiC/amorphous-C nanocomposites},
    volume = {80},
    issn = {23}
    shorttitle ={},
    url = {https://journals.aps.org/prb/abstract/10.1103/PhysRevB.80.235108},
    doi = {https://doi.org//10.1103/PhysRevB.80.235108},
    abstract = {The electronic structure of nanocrystalline (nc-) TiC/amorphous C nanocomposites has been investigated by soft x-ray absorption and emission spectroscopy. The measured spectra at the Ti 2p and C 1s thresholds of the nanocomposites are compared to those of Ti metal and amorphous C. The corresponding intensities of the electronic states for the valence and conduction bands in the nanocomposites are shown to strongly depend on the TiC carbide grain size. An increased charge transfer between the Ti 3d−eg states and the C 2p states has been identified as the grain size decreases, causing an increased ionicity of the TiC nanocrystallites. It is suggested that the charge transfer occurs at the interface between the nanocrystalline-TiC and the amorphous-C matrix and represents an interface bonding which may be essential for the understanding of the properties of nc-TiC/amorphous C and similar nanocomposites.},
    urldate = {2021-12-6},
    journal = {Physical Review B},
    author = {Magnuson, Martin and Lewin, Erik and Hultman, Lars and Jansson, Ulf},
    month = may,
    year = {2009},
    pages = {235108},
    file = {}
}

Class 1: disordered metal carbide films

in-text:
Often such disordered carbides
are not amorphous at the atomic scale but have a com-
posite microstructure of nanocrystalline transition metal
carbides embedded in amorphous graphite [22, 23]. 

--> 4,6,and 7 from the new references can be added to this statement, those papers concern nc-MC/a-C systems

Class 2:
In M-Si-C (M = Nb, Zr) systems, increase of Si
concentration above a critical concentration yields com-
pletely amorphous films [24, 25]. The mechanical and
electrical properties depend on the distribution of M-C,
M-Si and Si-C bonds [24, 25] in the amorphous phase. It
is further suggested that this class of amorphous transi-
tion metal carbides has an elastic modulus dependent on
the choice of transition metal [25].

